FAN: Foresight Action Normalization for Continual Adaptation of Vision-Language-Action Models

Vision-Language-Action (VLA) models pre-trained on large-scale, closed datasets have demonstrated remarkable success across diverse robotic manipulation tasks. However, their long-term real-world deployment necessitates continuously acquiring new skills while retaining previously learned capabilities. While pioneering works have explored continual VLA adaptation using techniques such as experience replay and reinforcement fine-tuning, they overlook a foundational mechanism: action normalization, which determines the underlying coordinate system in which policies perceive and execute physical actions. To bridge this gap, we systematically evaluate five normalization strategies across four real-world task streams covering single-arm and bimanual manipulation. Our analysis reveals that existing protocols induce severe failure modes due to inter-task coordinate drift, limited motion coverage, or train-test coordinate mismatches. Motivated by these insights, we formulate three core design principles: consistency, coverage, and causality (3C), and introduce foresight action normalization (FAN). FAN estimates normalization statistics once from a small, task-independent calibration set prior to continual learning and freezes them throughout adaptation. Across all evaluated streams, FAN achieves the highest performance and demonstrates consistent robustness, providing insightful guidance for building stable action representations in achieving effective lifelong VLA adaptation.

==> sections/0_abstract.tex <==
\begin{abstract}
AAAI creates proceedings, working notes, and technical reports directly from electronic source furnished by the authors. To ensure that all papers in the publication have a uniform appearance, authors must adhere to the following instructions.
\end{abstract}

==> sections/1_introduction.tex <==
Please serve as an expert in robot learning and continual learning to help write the paper entitled "RoboNever: A High-Quality Real-World Dataset for Continual Robot Learning." Now, read the materials and wait for my order. [[[Attached PDF files]]]

\section{Introduction}\label{sec:intro}

First, let's write the introduction section paragraph by paragraph. For the first paragraph, I would like to highlight that intelligent models, such as VLA models, have transformed robot learning into a new era. After that, we need to analyze the practical necessity of continual learning capabilities for VLA models. Ensure the writing is cohesive, concise, and professional, avoiding excessive sentence fragments.

Next, let's write the second paragraph. This paragraph will introduce 3-4 existing papers on continual learning of VLA models. Summarize each paper using 1-2 concise sentences. [[[Attached PDF files]]]

Then, let's write a new paragraph that comprehensively analyzes the issues in current studies and illustrates the necessity of our dataset. 

Finally, let's write the concluding paragraph summarizing our contributions. The contributions are threefold: 1) the dataset and various evaluation settings, 2) the attached training codebase, including implemented continual learning strategies, and 3) extensive experimental results.

Our contributions are threefold:
\begin{itemize}
    \item \textbf{High-quality dataset...}

    \item \textbf{Reproducible codebase...}

    \item \textbf{Extensive experiments...}
\end{itemize}


==> sections/2_related_work.tex <==
\section{Related Work}\label{sec:related_work}
\subsection{Robotic Manipulation}
Introduce the representative VLA models.

\subsection{Continual Robot Learning}
Introduce the current research on continual robot learning.

\subsection{Robotic Learning Datasets}
Introduce the representative robot learning datasets.

==> sections/3_background.tex <==
\section{Background}\label{sec:background}
\subsection{Markov Decision Process for Robot Learning}
\textcolor{red}{Please refer to the LIBERO paper.}

A robot learning problem can be formulated as a sequential decision-making problem. It can be described by a finite-horizon Markov Decision Process (MDP) defined by $\mathcal{M}=(\mathcal{S}, \mathcal{A}, P, R, \mu_0, H)$. Here, $\mathcal{S}$ and $\mathcal{A}$ denote the robot state space and action space, respectively.The transition function $P(s_{t+1}\mid s_t, a_t)$ describes how the environment evolves after executing action \(a_t\) in state \(s_t\), (R) is the reward function, \(\mu_0\) is the initial state distribution, and (H) is the task horizon. The goal is to learn a policy $\pi(a_t\mid s_t)$ that selects actions to maximize task performance over the horizon.

In real-world robot manipulation, however, the complete physical state is generally not directly observable. The robot can only access partial sensory observations, such as multi-view RGB images, proprioceptive states, end-effector poses, and gripper states. Therefore, we model real-world robot learning as a partially observable Markov Decision Process (POMDP) defined by $\mathcal{M}=(\mathcal{S}, \mathcal{O}, \mathcal{A}, P, \Omega, R, H)$. Here, $\mathcal{O}$ is the observation space, $\Omega(o_t\mid s_t,a_{t-1})$ is the observation function that generates an observation \(o_t\) from the underlying state.

Given an expert demonstration dataset $\mathcal{D}$, The goal of Robot Learning is to imitate the demonstrated actions by supervised fine-tuning the policy. The training objective is the negative log-likelihood loss:

\begin{equation}
L_{\mathrm{SFT}} =
\mathrm{E}{(o,a)\sim \mathcal{D}}
\left[
-\log \pi{\theta}(a \mid o,l)
\right].
\label{eq}
\end{equation}

where \(a\) is the expert action paired with observation \(o\), and \(l\) is the corresponding language-conditioned task instruction.

\subsection{Continual Robot Learning Problem}

\textcolor{red}{Formally define the robot learning process.}

We consider a task-incremental continual robot learning setting in which a single language-conditioned policy $\pi_{\theta}$ is trained over a sequence of \(K\) real-world manipulation tasks:
\begin{equation}
\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_K .
\label{eq}
\end{equation}

Each task $\mathcal{T}_k$ is associated with an expert demonstration dataset $\mathcal{D}_k = \left\{\tau_i^k\right\}_{i=1}^{N_k}$ and a language instruction \(l_k\). Each trajectory is represented as $\tau_i^{(k)} = \left\{(o_t^{(k)}, a_t^{(k)})\right\}_{t=0}^{H_i^{(k)}}$, where \(o_t^k\) denotes the multi-modal observation and \(a_t^k\) denotes the continuous robot action. The datasets arrive sequentially: when learning $\mathcal{T}_k$, the policy has full access to $\mathcal{D}_k$ and loses access to the previous k - 1 tasks.

For the (k)-th task, the supervised fine-tuning objective is
\begin{equation}
L_k =
\mathrm{E}_{(o,a)\sim \mathcal{D}k}
\left[
-\log \pi{\theta}(a \mid o,l_k)
\right].
\label{eq}
\end{equation}
The goal is to update one policy across the task stream such that, after learning $\mathcal{T}_k$, it performs well on all observed tasks ${\mathcal{T}_1,\ldots,\mathcal{T}_k}$.

To evaluate continual robot learning performance, we follow a task-sequence evaluation protocol. Let $\rho_{i,j}$ denote the normalized score on task $\mathcal{T}_i$ after the policy has been trained up to task $\mathcal{T}j$. In particular, $\rho{i,i}$ measures the performance on task $\mathcal{T}i$ immediately after it is learned, while $\rho_{i,K}$ measures the final retained performance on task $\mathcal{T}_i$ after the full task sequence has been completed.

\begin{equation}
\bar{\rho}_{K}
=
\frac{1}{K}
\sum_{i=1}^{K}
\rho_{i,K}.
\end{equation}
This metric summarizes the final capability of the policy across the entire task stream.

Negative backward transfer (NBT) quantifies forgetting on previously learned tasks:
\begin{equation}
\mathrm{NBT}{i} =
\frac{1}{K-i}
\sum{j=i+1}^{K}
\left(
\rho_{i,i} - \rho_{i,j}
\right),
\quad i<K.
\label{eq}
\end{equation}
A larger positive \(\mathrm{NBT}{i}\) indicates stronger forgetting, while a value close to zero indicates better retention of previously acquired skills.

\begin{equation}
\mathrm{FT}_{i}
=
\rho^{\mathrm{CL}}_{i,i}
-
\rho^{\mathrm{single}}_{i}.
\end{equation}
Here, $\rho^{\mathrm{single}}_{i}$ is the score obtained by training on \(\mathcal{T}_i\) alone. A positive \(\mathrm{FT}_{i}\) indicates beneficial transfer from previous tasks, whereas a negative value indicates reduced plasticity or interference during new-task learning.



==> sections/4_robonever.tex <==
\section{The RoboNever Dataset}\label{sec:robonever}
\textcolor{red}{Please refer to the RoboMind paper.}

\subsection{Robot Platform}
Introduce the detailed robot platform.

\subsection{Individual Task Design}

RoboNever contains ten real-world manipulation tasks designed to form heterogeneous continual learning benchmarks. The task suite is divided into two subsets: five single-arm tasks and five bimanual tasks. While the single-arm subset covers diverse primitive manipulation skills, the bimanual subset further introduces multi-object handling and arm coordination.

\textbf{Single-arm tasks.}
\begin{itemize}
    \item \textbf{Stack bowls:} grasp one bowl and stably stack it onto another bowl, evaluating pick-and-place accuracy and object alignment.
    \item \textbf{Hang cup:} grasp a cup and hang its handle on a rack without falling, emphasizing pose alignment and precise placement.
    \item \textbf{Press button:} press a round button vertically until activation, testing contact-rich precision control.
    \item \textbf{Fold towel:} fold a towel in half and adjust its edges, involving deformable object manipulation.
    \item \textbf{Push box:} push a box into a designated target region, focusing on non-prehensile manipulation and target reaching.
\end{itemize}

\textbf{Bimanual tasks.}
\begin{itemize}
    \item \textbf{Place cola:} use the two arms to grasp two cola cans and place both into a paper box, requiring sequential dual-arm object handling.
    \item \textbf{Cook bread:} manipulate bread and a pan with two arms; success requires placing the bread into the pan and moving the pan to the target location.
    \item \textbf{Place fruits:} place three fruits into a basket using both arms, evaluating repeated object transfer and bimanual task execution.
    \item \textbf{Fold T-shirt:} fold a T-shirt through coordinated dual-arm manipulation of a deformable garment.
    \item \textbf{Pack bag:} lift a paper bag into a carton and close the carton with both arms, requiring long-horizon bimanual coordination.
\end{itemize}

These subsets can be evaluated independently as single-arm and bimanual continual learning benchmarks, or combined into a mixed continual sequence.
.

\subsection{Data Collection}
Introduce the detailed processes of data collection, storage, and preprocessing.

\subsection{Evaluation Protocol}
Introduce the detailed evaluation protocol of each individual task.

\subsection{Training Configuration}
Introduce the optional training settings that comply with the continual learning scenario. For instance, train 5 single-arm tasks (inter-task) in a row, or train different modes of 1 task in a row (intra-task).

==> sections/5_experiments.tex <==
\section{Experiments}\label{sec:experiments}
In this section, we design experiments to investigate the following research questions:
\begin{itemize}
    \item \textbf{Q1:} 
    \item \textbf{Q2:} 
    \item \textbf{Q3:} 
\end{itemize}

\subsection{Experimental Setup}

\paragraph{Algorithmic Baselines.}
Introduce the implemented baselines, such as Pi0.5, experience replay, ewc, etc.

\paragraph{Evaluation Metrics.}
Formally define the metrics, such as the overall average success rate, negative backward transfer, and forward transfer.

\subsection{Results Analysis}
We conduct the following results analysis based on the pre-defined research questions.
\paragraph{Short summary 1 to respond/correlate the questions.}

\paragraph{Short summary 2 to respond/correlate the questions.}

\paragraph{Short summary 3 to respond/correlate the questions.}

==> sections/6_conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
One paragraph for summary.

One paragraph for (positive) limitations.
